Deep Learning From Four Vectors

An early example of the ability of deep networks to improve the statistical power of data collected in particle physics experiments was the demonstration that such networks operating on lists of particle momenta (four-vectors) could outperform shallow networks using features engineered with domain knowledge. A benchmark case is described, with extensions to parameterized networks. A discussion of data handling and architecture is presented, as well as a description of how to incorporate physics knowledge into the network architecture.

==> ws-rv9x6_2e/check.tex <==
%% Usage: Latex check.tex
%%
%% Utility to test if all the files required for wspc review volume project
%% are available in your present LaTeX path.
%% - ws-rv9x6.cls
%% - ws-crop9x6.sty
%% - crop.sty
%% - rotating.sty
%% - url.sty
%% - makeidx.sty
%% - chapterbib.sty
%% - cite.sty
%% - ws-minitoc.sty
%% - ws-index.sty

\newif\onerror

\typeout{*}
\typeout{1. Searching for LaTeX2e ... }
\ifx\documentclass\undefined
 \typeout{*}
 \typeout{* Fatal error occurred:}
 \typeout{*}
 \typeout{* The WS Review Volume class can only be used with LaTeX2e}
 \typeout{*}
 \typeout{* Stopping...}
 \expandafter\stop
\else
 \typeout{   ... ok}
\fi

\def\next#1/#2/#3\next{#1#2}
\typeout{ }
\typeout{2.  Searching for LaTeX2e version ... }
\ifnum\expandafter\next\fmtversion\next<199612 \relax
 \typeout{*}
 \typeout{* Fatal error occurred:}
 \typeout{*}
 \typeout{* Your LaTeX version is quite outdated, \fmtversion.}
 \typeout{* The WS Review Volume class can only be used with}
 \typeout{* a recent version of LaTeX2e, please upgrade your installation!}
 \typeout{*}
 \expandafter\stop
\else
 \ifnum\expandafter\next\fmtversion\next<199806 \relax
   \typeout{* Warning: }
   \typeout{*}
   \typeout{* Your LaTeX version is outdated, \fmtversion.}
   \typeout{* We believe that it will probably work, but if you encounter}
   \typeout{* problems you will need upgrade your installation.}
   \typeout{*}
   \typein{* Type <return> to continue ...}
   \errortrue
 \else
   \typeout{   ... ok}
 \fi
\fi

\typeout{ }
\typeout{3. Searching for ws-rv9x6.cls ... }
\IfFileExists{ws-rv9x6.cls}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{* ... ws-rv9x6.cls, file not found! }
     \typeout{*}
     \typeout{* Fatal error occurred:}
     \typeout{*}
     \typeout{* The ws-rv9x6 class file which is part of the WS Review Volume distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* Stopping...}
     \typeout{*}
     \stop
}

\typeout{ }
\typeout{4. Searching for ws-crop9x6.sty ... }
\IfFileExists{ws-crop9x6.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-crop9x6.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-crop9x6 file which is part of the WS Books distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* Without this package you will not be able to typeset }
     \typeout{* your book in 9x6 trim size.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{5. Searching for crop.sty ... }
\IfFileExists{crop.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... crop.sty, file not found! }
     \typeout{*}
     \typeout{*}
     \typeout{* The crop package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* This package is required for printing the crop marks.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "crop".}
     \typeout{*}
     \typeout{* Stopping...}
     \typeout{*}
     \stop
}

\typeout{ }
\typeout{6. Searching for rotating.sty ... }
\IfFileExists{rotating.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... rotating.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The rotating package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to use}
     \typeout{* sidewaysfigure and sidewaystable environments.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "rotating".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{7. Searching for url.sty ... }
\IfFileExists{url.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... url.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The url package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to use the \string\url}
     \typeout{* command. Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "url".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{8. Searching for makeidx.sty ... }
\IfFileExists{makeidx.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... makeidx.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The makeidx package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to generate index.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "makeidx".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{9. Searching for chapterbib.sty ... }
\IfFileExists{chapterbib.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... chapterbib.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The chapterbib package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to include separate bibliography for each chapter.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "chapterbib".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{10. Searching for cite.sty ... }
\IfFileExists{cite.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... cite.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The cite package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to generate citations in superscript.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "cite".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{11. Searching for ws-minitoc.sty ... }
\IfFileExists{ws-minitoc.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-minitoc.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-minitoc package which is part of the WS Review Volume distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* You can use the ws-rv9x6 class without this package but }
     \typeout{* you can not have chapter level tocs.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{12. Searching for ws-rv-har.bst ... }
\IfFileExists{ws-rv-har.bst}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-rv-har.bst, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-rv-har bibliography style file which is part of the WS Review Volume distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* You can use the ws-rv9x6 class without this package but }
     \typeout{* you can not use BiBTeX features.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{13. Searching for ws-rv-van.bst ... }
\IfFileExists{ws-rv-van.bst}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-rv-van.bst, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-rv-van bibliography style file which is part of the WS Review Volume distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* You can use the ws-rv9x6 class without this package but }
     \typeout{* you can not use BiBTeX features.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{14. Searching for ws-index.sty ... }
\IfFileExists{ws-index.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-index.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-index package which is part of the WS RV distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* You can use the ws-rv9x6 class without this package but }
     \typeout{* you can not use multiple indexes.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{* Finished Testing *}
\typeout{ }
\onerror
\typeout{* Some of the files/packages required by WS was not found,}
\typeout{*}
\typeout{* Please review the above comments carefully and update your system.}
\typeout{*}
\typeout{*****************************************************************}
\typein{* Type <return> to continue ...} \else
\typeout{******************************************************}
\typeout{*}
\typeout{* All the files and packages required by WS was found,}
\typeout{* you may now proceed LaTeXing your files.}
\typeout{*}
\typeout{******************************************************} \fi
\stop
\endinput

